JavaVFC: Java Vulnerability Fixing Commits from Open-source Software

We present a comprehensive dataset of Java vulnerability-fixing commits (VFCs) to advance research in Java vulnerability analysis. Our dataset, derived from thousands of open-source Java projects on GitHub, comprises two variants: JavaVFC and JavaVFC-extended. The dataset was constructed through a rigorous process involving heuristic rules and multiple rounds of manual labeling. We initially used keywords to filter candidate VFCs based on commit messages, then refined this keyword set through iterative manual labeling. The final labeling round achieved a precision score of 0.7 among three annotators. We applied the refined keyword set to 34,321 open-source Java repositories with over 50 GitHub stars, resulting in JavaVFC with 784 manually verified VFCs and JavaVFC-extended with 16,837 automatically identified VFCs. Both variants are presented in a standardized JSONL format for easy access and analysis. This dataset supports various research endeavors, including VFC identification, fine-grained vulnerability detection, and automated vulnerability repair. The JavaVFC and JavaVFC-extended are publicly available at https://zenodo.org/records/13731781.

==> background.tex <==
\section{Background}
% The identification and fixing of software vulnerabilities are crucial processes in ensuring the security and reliability of software systems. As software projects grow in complexity, the potential for introducing security vulnerabilities increases, necessitating the development of effective tools and methods for detecting and mitigating these issues. The process of identifying vulnerabilities often involves analyzing code changes in repositories, where developers fix identified issues and improve the security posture of their software.

% Java, as one of the most widely used programming languages, plays a significant role in enterprise applications and open-source projects. The popularity of Java is reflected in the vast number of repositories hosted on platforms like GitHub, where developers collaborate, share, and improve code. GitHub, being the largest platform for open-source software development, provides a rich source of data for studying how vulnerabilities are introduced and fixed in real-world projects.

Our dataset is designed to address the need for high-quality, real-world data that can be used to train and evaluate vulnerability detection tools. By focusing on Java repositories with significant community engagement, we aim to capture a diverse and representative sample of software projects that reflect real-world practices. This dataset not only facilitates the development of more accurate vulnerability detection models but also provides insights into the patterns and practices associated with fixing vulnerabilities in software projects.

\subsection{Potential research opportunities using this dataset}
Security vulnerabilities in software are a critical concern for developers and organizations alike. Addressing these challenges requires advancements in areas such as vulnerability detection, vulnerability fixing commits detection, and code quality. Our curated dataset offers a foundation for future research in several potential areas, including but not limited to the following:

\subsubsection{Vulnerability Detection} The dataset can be instrumental in advancing the state of security vulnerability detection in software. It enables the exploration of patterns in vulnerable code changes, which can lead to the development of more sophisticated machine learning models for vulnerability detection. Researchers can investigate how different types of vulnerabilities manifest in code and how they are typically addressed by developers in real-world projects. The dataset also provides opportunities to study the effectiveness of various vulnerability detection tools by benchmarking them against real-world commits, thus helping to improve their accuracy and reliability.

\subsubsection{Vulnerability Fixing Commits Detection} The dataset can support research aimed at detecting which commits are likely to fix vulnerabilities. By analyzing historical commits and associated metadata, researchers can develop models that identify potential vulnerability-fixing commits based on patterns in code changes, commit messages, and project characteristics. These models could be integrated into continuous integration pipelines to help developers identify and prioritize critical fixes, ultimately improving the security and stability of software projects.

\subsubsection{Empirical Studies} The dataset facilitates empirical studies on the process of fixing vulnerabilities in software. Researchers can analyze the methods and approaches used by developers to fix vulnerabilities, identifying common patterns and best practices. These studies could also investigate the impact of developer expertise and project characteristics on the effectiveness of vulnerability fixes, providing insights that could improve the training and support provided to developers.
